Spy in the GPU-box: Covert and Side Channel Attacks on Multi-GPU Systems

The deep learning revolution has been enabled in large part by GPUs, and more recently accelerators, which make it possible to carry out computationally demanding training and inference in acceptable times. As the size of machine learning networks and workloads continues to increase, multi-GPU machines have emerged as an important platform offered on High Performance Computing and cloud data centers. As these machines are shared between multiple users, it becomes increasingly important to protect applications against potential attacks. In this paper, we explore the vulnerability of Nvidia's DGX multi-GPU machines to covert and side channel attacks. These machines consist of a number of discrete GPUs that are interconnected through a combination of custom interconnect (NVLink) and PCIe connections. We reverse engineer the cache hierarchy and show that it is possible for an attacker on one GPU to cause contention on the L2 cache of another GPU. We use this observation to first develop a covert channel attack across two GPUs, achieving the best bandwidth of 3.95 MB/s. We also develop a prime and probe attack on a remote GPU allowing an attacker to recover the cache hit and miss behavior of another workload. This basic capability can be used in any number of side channel attacks: we demonstrate a proof of concept attack that fingerprints the application running on the remote GPU, with high accuracy. Our work establishes for the first time the vulnerability of these machines to microarchitectural attacks, and we hope that it guides future research to improve their security.

==> Reverse-Eng.tex <==
\section{Reverse Engineering Cache Organization}\label{sec:Reverse-Eng}
\nael{I flipped the order of the two subsections since there is a chicken and egg problem.  If you dont know where the remote data is cached, then how can you do the timing experiments?  However, later I noticed that the caching policy section relies on the timing thresholds that you get from the timing subsection.  So, there is a circular dependency between the two.}
\nael{ Definitely, the old order does not work since the first experiment provided more information than the second.  To me the timing section is sufficient to reverse engineer both questions -- you show that you have 4 levels of delays corresponding to locally mapped vs. remotely mapped cache sets.  There is no need for Algorithm 1 and Figure 4, and we can consolidate everything.  I am not making that change now, but let us discuss. }

%%\item {\bf Local and remote access time:}
%To conduct the attack from the remote GPU, the attacker needs to resolve the local and remote GPU access time. To distinguish the hits and misses while accessing the local and remote GPUs is imperative to determine the cache sets and also to conduct the attack. We conducted an experiment to determine the local and remote access times.
   
%\item{\bf Caching mechanism in multi-GPU system:}
In multi-GPU system, a GPU can access the memory of a remote GPU that is connected via NVLink. The caching organization as seen through this GPU-to-GPU communication is the primary mechanism we use in our attacks.  However, since it is not documented, we had to reverse engineer its behavior to be able to conduct successful attacks.  %Specifically, when the data gets cached in both remote and local GPUs, the attacker needs to evict the data from the cache of local GPU to measure the access time in the remote cache. %Through our experiment we determined that the data gets cached only in the remote GPU.
In this section, we present the experiments and findings that we used to understand this caching mechanism.  % conducted some experiments to understand the caching mechanism for accesses to a remote GPU. 

%\nael{The next paragraph is not clear; how/why would you use these APIs?  Dont you access the remote device simply by accessing a memory page mapped to it?  What is the higher level point being made here?}
%\sankha{The next paragraph just explains the nvidia provided apis through which you can pin the current gpu device and then how you can access the remote gpu}\nael{Help me understand, please: Access what/how on a remote GPU?  access it to launch kernels on it, or access memory mapped to it?  What does it mean to access a peer device?  What is the granularity and of what resources?  The description is very cryptic and I am not sure how to revise it to make the point you want to make: what do you want to say at a high level?  Does the enable peer access mean that victim has to cooperate to enable the other process access to the remote GPU?  I see the commented out text below this (I dont remember, maybe I commented it out) but it does not answer my questions clearly either).  Also, perhaps this is something that can go in threat model since it is related to access.}\nael{I see these are introduced later as part of the cache hit/miss timing, so probably best to comment them out here.}

%Nvidia provides APIs that allow a user to select the GPU they execute a kernel on.  These include \textit{cudaSetDevice(\textit{devID})} to set the current GPU where \textit{devID} specifies the current GPU ID to be used. APIs like \textit{cuadDeviceEnablePeerAccess(peerDevice,flags)} are also provided to access a peer device that is connected via NVLink. The \textit{peerDevice} variable specifies the peer device that the user wants to access. %If the \textit{peerDevice} is not connected via NVLink, then this API returns error. 
%In our experiments, we used CUDA provided \textit{clock()} function to measure the access time. 


%Considering a situation similar to depicted in Fig. \ref{fig:threatModel_1}, if an attacker wants to find local L2 hit and miss time, attacker first specifies the current device using \textit{cudaSetDevice}. So if the local device is GPU A, then attacker would allocate a buffer on the local device on GPU A. To measure remote L2 hit and miss time, like the spy process, needs to set the remote GPU A as the current GPU to allocate a buffer first on the remote GPU. Then the current GPU needs to be changed to set to GPU B and enable the access to the remote GPU A using \textit{cuadDeviceEnablePeerAccess}. Now, that we have a clear understanding about local and remote GPU access methodology.

\subsection{Reverse Engineering Caching Policy in Multi-GPU systems}

In the first set of experiments, our goal is to understand how data gets cached within a multi-GPU system.  The DGX-1 offers a uniform address space, and virtual pages can be allocated to physical pages that belongs in any of the GPU HBM DRAM memory.  Our goal is to understand how accesses to data gets cached among the different GPUs.  Pascal GPUs have two levels of data cache, L1 and L2. A programmer can bypass L1 data caching by using specific data loading primitives like \textunderscore\textunderscore\textit{ldcg()}. However, L2 data caching cannot be bypassed and all data and instructions get cached in L2. 

\begin{figure}[htbp]
    \centering
   \vspace{-0.2in}
    \includegraphics[width=.95\linewidth, height=0.8\linewidth]{Figs/ThreatModel.png}
    \caption{Accessing a remote GPU's memory through NVLink}
    \vspace{-0.1in}
    \label{fig:threatModel_1}
\end{figure}

 The access pathways to DRAM (local and remote) are shown in Figure~\ref{fig:threatModel_1}.  When DRAM pages are allocated in the local GPU memory, the data access path is straightforward: the first access is serviced from DRAM and the subsequent accesses hit the L2 cache on the same device.  On the other hand, when the data is allocated on one GPU and accessed from another, the request is routed through the NvLink connection and the requested cache line is also sent back through NvLink.  Our goal is to determine where the data gets cached  (local or remote L2 cache).   Of course, caching the data locally, would introduce cache coherence issues since copies of the same data could exist in multiple L2 caches.  %then there are three scenarios that could arise. Data could be cached in L2 caches of both the devices, or only in the L2 cache of local GPU, or only in the L2 of the remote GPU. We conducted an experiment to determine the caching mechanism in multi-GPU environment that is shown in Algorithm \ref{alg:accessPath}. 
\nael{Is this information available in data sheets or whitepapers?}

\begin{small}
\begin{algorithm}
\SetAlgoLined
\For{$i = 0;\ i < numOfAccessRepeats;\ i = i + 1$}{\label{alg:pathLn_1} 
    \textit{startIdx} = \textit{fixedIdx};\\\label{alg:pathLn_2} 
    ptr = \&dataBuffer[startIdx];\\\label{alg:pathLn_3} 
    start = clock();\\\label{alg:pathLn_4} 
    startIdx = \textunderscore\textit{ldcg(ptr)};\\\label{alg:pathLn_5} 
    dummy = dummy + startIdx;\\\label{alg:pathLn_6} 
    end = clock();\\\label{alg:pathLn_6} 
    shareBuff[i] = (start-end);\\\label{alg:pathLn_7} 
    \textunderscore\textunderscore\textit{threadfence()};\label{alg:pathLn_8} 
}\label{accessLn_9}
%\textit{dummy operations to prevent compiler optimizations};\\\label{alg:pathLn_10} 
\textit{copy shared time buffer to main time buffer};\\\label{alg:pathLn_11} 

\caption{Remote GPU Access Microbenchmark}
\label{alg:accessPath}
\end{algorithm}
\end{small}

\begin{figure}[htbp]
    \centering
    \vspace{-0.1in}
    \includegraphics[width=\linewidth,height=.3\linewidth]{Figs/RemDevCaching.jpg}
    \caption{Timing remote GPU caching}
    \label{fig:accessPath}
    \vspace{-0.12in}
\end{figure}

%Consider a situation demonstrated in Fig \ref{fig:threatModel_1} when two GPUs are connected via NVLink. 
 We used the microbenchmark shown in Algorithm~\ref{alg:accessPath} to determine the answer to this question.  A data buffer \textit{dataBuffer} is allocated on a remote \textit{GPU A} and a kernel is launched from \textit{GPU B}.  Lines \ref{alg:pathLn_1} - \ref{accessLn_9} access the same piece of data for \textit{numOfAccessRepeats} number of times. The first access will be served from the DRAM and the subsequent accesses will be serviced from the L2 cache. Line \ref{alg:pathLn_2}, indicates the fixed index of the buffer specified by the user that is being accessed repeatedly. %The date is accessed in \ref{alg:pathLn_5} by de-referencing the pointer and \ref{alg:pathLn_6} is a dummy operation to avoid the compiler optimization. The access cycles is recorded in \ref{alg:pathLn_7} in the shared buffer. 
We repeat this experiment several times, clearing the cache between experiments.   If the data gets cached on both local and remote GPU L2 cache or in local GPU L2 cache, we will see the local L2 cache access time for subsequent accesses. %in line \ref{alg:pathLn_5} within the loop. 
However, if the data is only cached in the remote L2 GPU cache, we will only see remote L2 cache access cycles in the subsequent accesses within the loop. Figure \ref{fig:accessPath} shows the access cycles of our experiment.



We called the kernel for 20 times and our \textit{numOfAccessRepeats} is 4. So the first access is the DRAM access and the consecutive three accesses would be serviced from the L2 cache. As the data is accessed remotely, the DRAM access is above 800 cycles which was expected. However, the timing results show that the consecutive three accesses were serviced from the remote L2 cache with an access cycle above 600. %The first access of the first kernel launch is always higher than all other accesses for the device initialization. 
\textbf{In summary, our reverse engineering results demonstrate that an access to the memory of a remote GPU through NVLink is cached on the L2 cache of remote GPU, but not L2 cache of local GPU.}
As our reverse engineering results show that the data gets cached on remote GPU L2 cache only, no explicit eviction is required on the local GPU. We use this shared remote L2 cache in GPU-to-GPU communication to build microarchitectural covert and side channel attacks. Fig. ~\ref{fig:threatModel_1} shows our threat model and the data path to access a remote GPU’s memory through NVLink. 

%GPU caches are non-inclusive and the NVidia doesn't provide any special instruction to clear the cache levels (like \textit{CLFLUSH} in x86 architecture). So an attacker can take advantage of this form of remote caching in the multi-GPU scenario to develop attacks. Because if the data gets cached in the local L2 cache as well, then the attacker has to evict the target data from the local L2 cache to reach the remote L2 cache during the actual attack. However, our reverse engineering results show that no such explicit eviction is required on the local GPU. We use this shared remote L2 cache in GPU-to-GPU communication to build microarchitectural covert and side channel attacks. Figure~\ref{fig:threatModel_1} shows our threat model and the data path to access a remote GPU’s memory through NVLink. 


\subsection{Timing characteristics of local and remote accesses}

In traditional cache-based timing attacks, an attacker needs to distinguish the cache hit and miss time for different cache levels in order to identify data/cache sets being accessed by the other process (either as part of a covert or side channel attack). %However, conventional Prime+Probe based cache timing attacks are conducted within a single component and understanding the access times of all cache level within the component is sufficient to conduct the attack. 
In our cross-GPU L2 based timing attack, the attacker needs to determine the hit and miss time of both local and remote GPU's caches. Since our attack relies on creating contention between a remote GPU and a local GPU, we developed a microbenchmark to determine the access time of local and remote L2 cache hits and misses. %\nael{Perhaps it would help to have seen Figure 5 before this?  At this point, the reader will have to take it for granted that "determining the time of local and remote L2 cache hits and misses" is what we need.  Alternatively, you can add a forward reference (e.g., "we will show later that the attacker ...")} %shown in Algorithm \ref{alg:accessTime}.
\begin{comment}
\begin{small}
\begin{algorithm}
\SetAlgoLined
\textit{startIdx} = 0;\\\label{accessLn_1}
\For{$i = 0;\ i < numEls;\ i = i + 1$}{ \label{accessLn_2}
    ptr = \&dataBuffer[startIdx];\\\label{accessLn_3}
    start = clock();\\\label{accessLn_4}
    startIdx = \textunderscore\textunderscore\textit{ldcg(ptr)};\\\label{accessLn_5}
    dummy = dummy + startIdx;\\\label{accessLn_6}
    end = clock();\\\label{accessLn_7}
    shareBuff[i] = (start-end);\\\label{accessLn_8}
    \textunderscore\textunderscore\textit{threadfence()};\\\label{accessLn_9}
}\label{accessLn_10}

\textit{dummy operations};\\\label{accessLn_11}
\textit{startIdx} = 0;\\\label{accessLn_12}

\For{$i = 0;\ i < numEls;\ i = i + 1$}{\label{accessLn_13} 
    ptr = \&dataBuffer[startIdx];\\
    start = clock();\\
    startIdx = \textunderscore\textit{ldcg(ptr)};\\
    dummy = dummy + startIdx;\\
    end = clock();\\
    shareBuff[numEls+i] = (start-end);\\
    \textunderscore\textunderscore\textit{threadfence()};
}\label{accessLn_14}

\textit{dummy operations};\\
\textit{copying shared time buffer to main time buffer};\\

\caption{Access Time Kernel Algorithm}
\label{alg:accessTime}
\end{algorithm}
\end{small}
\end{comment}

%\hoda{I think we can remove Algorithm 1 (and probably some other algorithms) and explain it very briefly in text to save some space. I keep it for now. We have 5 algorithms in the paper so far. Can we put all of them in an Appendix? I am not sure if they allow appendix in the submission, though!}
%\sankha{We can this one but then explanation would needed to be verbose. Also I am concerned that removing the algorithm would make the explanation confusing to the reviewers. Moving the algos to the appendix should be fine. Let me check if we can.}
We allocate a buffer in the memory of one of the GPUs and use accesses to it to derive both local and remote access times.  To find both the remote and local access time, we %can use the kernel shown in  Algorithm \ref{alg:accessTime}. There are two loops in the algorithm. The first loop from line \ref{accessLn_2}-\ref{accessLn_10} 
first populate the L2 cache with the data from a buffer in DRAM with the stride of 128 bytes which is the L2 cache line size for our Pascal 100 GPU architecture. %First the start index needs to be specified which is set to 0 as shown in line \ref{accessLn_1}. The range of the number of elements needs to be accessed is specified in \textit{numEls} in line \ref{accessLn_2}. The data access takes place in Line \ref{accessLn_5} where we are de-referencing the pointer to access the data. 
We use the \textunderscore\textunderscore\textit{ldcg()} load primitive to load the data which allows the data to get cached in the L2 cache only and avoids L1 caching. Each data access is followed by a dummy operation %in line \ref{accessLn_6} 
to make sure the access is not optimized out by the compiler. %The data access time and the dummy operations are encapsulated within two clock functions. %The first clock function is called in line \ref{accessLn_4} which records the start of the operation and the next clock function in line \ref{accessLn_7} records the end of the operation. The difference 
The access time is measured using the clock() function and is recorded in a shared buffer %in line \ref{accessLn_8} 
to avoid any contention in the L2 cache as the access path of the shared buffer is separate than the main memory access path. This first cold access shows the DRAM access time. We access the buffer again and measure the access time which represents the L2 cache access time.

%The second loop from line \ref{accessLn_13} to \ref{accessLn_14} is exact similar to the previous loop. But the access in the second loop takes place in the L2 cache as the data is already cached and the time recorded in this section of the loop gives the L2 cache access time. 

\begin{figure}[htbp]
    %\centering
  \vspace{0.1in}
    \includegraphics[width=1\columnwidth]{Figs/dataAccessTime.jpg}
    \caption{Local and remote GPU access time}
    \label{fig:accessTime}
    \vspace{-0.1in}
\end{figure}

If we want to find \textit{local} L2 hit and miss time, we first specify the current device using \textit{cudaSetDevice}. So if the local device is GPU A, then we allocate a buffer on the local device on GPU A. To measure \textit{remote} L2 hit and miss time, we need to set the remote GPU A as the current GPU to allocate a buffer first on the remote GPU. Then the current GPU needs to be changed to GPU B and we are able to access to the remote GPU A using \textit{cudaDeviceEnablePeerAccess}.

The local and remote GPU L2 and DRAM access time is shown in Fig \ref{fig:accessTime} histogram. We have made 48 accesses in each loop to measure both local and remote GPU. The X-axis specifies the access delay of the data and the Y axis specifies the number of bins in the histogram. As it is shown, the L2 cache hits and misses for both local and remote accesses are clearly distinguishable. %The access time in different scenarios are provided in Table \ref{tab:accessTime}. %As we can see that the access cycles in DRAM and L2 cache are pretty discernible in local and remote GPUs. 
%\nael{This table can be removed if we need space since the information is already visible in Figure 3}
\begin{comment}
\begin{table}
\centering
\caption{Access Cycles in Local and Remote GPU}
\begin{tabular}{ |c|c| } 
\hline
\textbf{Data Access Type} &  \textbf{Access Cycles}\\ 
\hline
Local L2 Cache   & $240\le x \le 300$ \\  
\hline
Local DRAM   & $420\le x \le 520$ \\ 
\hline
Remote  L2 Cache   & $600\le x \le 700$ \\  
\hline
Remote DRAM   & $800\le x$ \\ 
\hline
\end{tabular}

\label{tab:accessTime}
\vspace{-0.20in}
\end{table}
\end{comment}



==> sidechannel.tex <==
\section{Application Fingerprinting Classifier}

%\nael{ML is just a tool here to classify the output of the attack.  Focus should be on side channel attack.}

%\nael{Emphasis is still on the classifier.  The contribution is the side channel attack, not the classifier.  Its standard to use machine learning to infer data in a side channel attack, so emphasis is totally on the wrong thing in my opinion (the tool to recover information, rather than the fact that information is leaking).  Starts from the title, and then goes through the description.}
%\hoda{Yes, the title of this section will be "side channel attacks". Sankha hasn't started writing this section yet. Now just the ML classification is there, but details of side channel attack will be added at the start of this section later.}

Deep learning has seen a meteoric rise in the last decade due to the increased computational capabilities of modern computers combined with the vast amount of information available to facilitate learning \cite{manel_book} \cite{Goodfellow}. Deep learning provides a framework for data based learning approaches and can extract increasingly abstract features from the data. A particular class of deep learning framework known as the Convolutional Neural Networks (CNN) has revolutionised the field of computer vision and visual learning \cite{LeNet} \cite{alexnet} \cite{vgg}. Residual Networks (ResNet) introduced by He et al. utilizes residual connections every two layers of a CNN to reduce training time and provide superior generalization in classification tasks such as image recognition and detection, segmentation, text understanding and a host of other computer vision and artificial intelligence tasks \cite{resnet}. Resnets are not limited to a particular size of the image data which it was trained on, it can readily adapt to an image data of any shape which allows for transfer learning and fast retraining to a changing observation scenario.

In this paper we harness the power of deep learning frameworks and utilize them for application fingerprinting by constructing a one vs all classifier to classify the processes running on the GPU. We formulate the application fingerprinting problem as a computer vision task and use the extracted frames from microarchitectural attack to teach the machine to detect which application is currently being executed on the GPU. 

\subsection{Classifier Architecture}

This paper employs a variant of the ResNet composed of 18 successive layers with residual connections known as the Resnet18. The networks weights were pretrained on ImageNet dataset which has a total of 14,197,122 images \cite{imagenet}. ResNet employs full $3 \times 3$ convolutional layer design for each block of convolutions. Each residual block has two stacked $3 \times 3$ convolutional layers with equal number of outputs and every convolutional layer is followed by a batch normalization layer and employs a ReLU (Rectified Linear Unit) activation function. The output from each block is then added to the input to the block before the final ReLU activation function. The pretrained ResNet18 head is followed by a fully connected layer with the number of nodes equivalent to the number of classes in the application dataset generated using the side channel attack described in section \ref{}. Since the output can be any one of the six possible applications running on the GPU, we apply a Categorical Crossentropy loss function to facilitate multi-class classification and a Stochastic Gradient Descent Optimizer (SGD) to optimize the network parameters with a learning rate of $1e^{-4}$ \cite{sgd2016}. We hypothesize that a ResNet18 pretrained to execute image recognition will facilitate transfer learning and the machine will be able to generalize well across the six classes with few shot learning \cite{transfer_learning1} \cite{transfer_learning2}. Since the network weights have been optimized on image classification tasks it should aid convergence and we can achieve good accuracy on application classification. 

\subsection{Data and Performance}
The data set to train and evaluate the classifier is composed of $1500$ samples from the six classes, one for each application in Black Schole, Histogram, Matrix Multiplication, Quasi Random Number generator, Vector Addition and Welsh Transform. Since the amount of data is rather small for a computer vision problem we attempt few shot learning to train it. having pretrained the resnet on image recognition tasks, we split the data into training and validation sets of 150 samples each and isolate $1200$ samples as the test or control set. Since there is no class imbalance in the data set, keeping a sufficiently large test set ensures that we evaluate the generalization capabilities of the machine with good confidence.

\begin{table}[h!]
\centering
\caption{Test Accuracy}
\begin{tabular}{ |c|c| } 
\hline
\textbf{Application [Class]} &  \textbf{Test Accuracy [\%]}\\ 
\hline
Black Schole   &  100\% \\  
\hline
Histogram   & 99.75\% \\ 
\hline
Matrix Multiplication   & 100\%  \\  
\hline
Quasi Random Generator   & 100\%  \\ 
\hline
Vector Addition & 100\% \\
\hline
Welsh Transform   & 99.91\% \\ 
\hline
\end{tabular}

\label{tab:accuracy}
\end{table}

The ResNet architecture employed for application classification achieved an overall accuracy of $99.91\%$ on the test set of $7200$ samples spanning six classes. Since there is no class imbalance in the data, this provides sufficient evidence that the machine is able is generalize very well on the task of application classification. Table \ref{tab:accuracy} shows the classification accuracy of each of the individual classes (applications) considered for this research. Black Schole, Matrix Multiplication, Quasi Random Generator and Vector Addition was able to achieve a perfect accuracy score of $100\%$ while Histogram and Welsh Transform scored $99.75\%$ and $99.91\%$ respectively. The confusion matrix depicting the classification results is shown in Figure \ref{fig:confusion_matrix}. The results vindicate the use of computer vision techniques for side channel application fingerprinting. Moreover, the formulation can be readily extended to classify a larger number of applications.
\begin{figure}
    \centering
    \vspace{-0.2in}
    \includegraphics[width=\linewidth]{Figs/confusion_matrix.png}
    \caption{Confusion Matrix as obtained for the test set with 1200 samples for each class where BS is Black Schole, HG is Histogram, MM is Matrix Multiplication, QR is Quasi Random generator, VA is Vector Addition and WT is Welsh Transform.}
    \label{fig:confusion_matrix}
    \vspace{-0.2in}
\end{figure}

